A novel local search based on variable-focusing for random K-SAT

We introduce a new local search algorithm for satisfiability problems. Usual approaches focus uniformly on unsatisfied clauses. The new method works by picking uniformly random variables in unsatisfied clauses. A Variable-based Focused Metropolis Search (V-FMS) is then applied to random 3-SAT. We show that it is quite comparable in performance to the clause-based FMS. Consequences for algorithmic design are discussed.

==> refs.tex <==
\bibitem{AaLe97}
E. Aarts and J. K. Lenstra (Eds.),
Local Search for Combinatorial Optimization.
J. Wiley \& Sons, New York NY, 1997.

\bibitem{AA06}
J. Ardelius and E. Aurell,
Behavior of heuristics on large and hard satisfiability problems.
Phys.\ Rev.\ E 74 (2006) 037702.

\bibitem{AGK05}
E. Aurell, U. Gordon, and S. Kirkpatrick.
Comparing beliefs, surveys and random walks.
Advances in Neural Information Processing Systems 17 (NIPS-04),
49--56. The MIT Press, 2005.

\bibitem{BaHW03}
W. Barthel, A. K. Hartmann, and M. Weigt,
Solving satisfiability problems by fluctuations: The dynamics
of stochastic local search algorithms.
Phys.\ Rev.\ E 67 (2003) 066104.

\bibitem{Battaglia-etal05}
D. Battaglia, A. Braunstein, J. Chavas, and R. Zecchina,
Source coding by efficient selection of ground-state clusters,
Phys.\ Rev.\ E 72 (2005) 015103.


\bibitem{DuGP97}
D. Du, J. Gu, P. Pardalos (Eds.),
Satisfiability Problem: Theory and Applications.
DIMACS Series in Discr.\ Math.\ and Theoret.\ Comput.\ Sci.\ 35,
American Math.\ Soc., Providence RI, 1997.

\bibitem{DMSZ01}
O. Dubois, R. Monasson,
B. Selman and R. Zecchina (Eds.).
Special Issue on NP-Hardness and Phase Transitions.
Theoret.\ Comput.\ Sci.\ 265 (2001).


\bibitem{GaJo79}
M. R. Garey and D. S. Johnson,
Computers and Intractability: A Guide to the Theory of NP-Completeness.
W. H. Freeman \& Co., San Francisco CA, 1979.

\bibitem{HoSt05}
H. H. Hoos and T. St\"utzle,
Stochastic Local Search: Foundations and Applications.
Morgan Kaufmann (Elsevier), 2005.


\bibitem{KaSe07}
H. Kautz and B. Selman.
The state of SAT. Discrete Appl. Math. 155 (2007) 1514--1524.

\bibitem{KGV83}
S. Kirkpatrick, C. D. Gelatt, Jr., and M. P. Vecchi,
Optimization by simulated annealing, Science 220 (1983) 671--680.


\bibitem{KrSS07}
L.~Kroc, A.~Sabharwal, and B.~Selman.
Survey propagation revisited.
Proceedings, 23rd Conference on Uncertainty in Artificial
Intelligence (UAI-07), 217--226.
AUAI Press, Arlington, Virginia, 2007.

\bibitem{KrMR07}
F. Krzakala, A. Montanari, F. Ricci-Tersenghi, G. Semerjian, and L. Zdeborova,
Gibbs states and the set of solutions of random constraint
satisfaction problems. Proc. Nat. Acad. Sci. USA 104 (2007)
10318--10323.

\bibitem{MMZ01}
O. C. Martin, R. Monasson, and R. Zecchina,
Statistical mechanics methods and phase transitions in
optimization problems,
Theoret.\ Comput.\ Sci.\  265 (2001) 3--67.


\bibitem{MeMZ06}
S. Mertens, M. M\'ezard, and R. Zecchina,
Threshold values for random $K$-SAT from the cavity method,
Random Structures Algorithms 28 (2006) 340--373.

\bibitem{MeMZ05}
M. M\'ezard, T. Mora, and R. Zecchina,
Clustering of solutions in the random satisfiability problem,
Phys.\ Rev.\ Lett.\ 94 (2005) 197205.

\bibitem{MPZ02}
M. M\'ezard, G. Parisi, and R. Zecchina,
Analytic and algorithmic solutions of random satisfiability problems.
Science 297 (2002) 812--815.

\bibitem{MiSL92}
D. Mitchell, B. Selman, and H. Levesque,
Hard and easy distributions of SAT problems.
Proc.\ 10th Natl.\ Conf.\ on Artificial Intelligence (AAAI-92),
459--465. AAAI Press, San Jose CA, 1992.

\bibitem{MM97}
R. Monasson and R. Zecchina,
Statistical mechanics of the random $K$-SAT problem.
Phys.\ Rev.\ E 56 (1997) 1357--1361.

\bibitem{MoPR04}
A. Montanari, G. Parisi, and F. Ricci-Tersenghi,
Instability of one-step replica-symmetry-broken phase in
satisfiability problems,
J.\ Phys.\ A 37 (2004) 2073--2091.

\bibitem{Papa91}
C.H. Papadimitriou,
On selecting a satisfying truth assignment.
Proc.\ 32nd IEEE Symposium on the Foundations of Computer
Science (FOCS-91), 163--169.
IEEE Computer Society, New York NY, 1991.

\bibitem{Pari02}
G. Parisi,
On local equilibrium equations for clustering states.
Technical report cs.CC/0212047, arXiv.org (Feb 2002).

\bibitem{SeAO05}
S. Seitz, M. Alava, and P. Orponen,
Focused local search for random 3-satisfiability,
J.\ Stat.\ Mech.\ Theory Exp.\ (2005) 06006.

\bibitem{SeKC96}
B. Selman, H. Kautz, and B. Cohen,
Local search strategies for satisfiability testing.
In: D. S. Johnson and M. A. Trick (Eds.),
Cliques, Coloring, and Satisfiability, 521--532.
DIMACS Series in Discr.\ Math.\ and Theoret.\ Comput.\ Sci. 26,
American Math.\ Soc., Providence RI, 1996.

\bibitem{SKM97}
B. Selman, H. Kautz, and D. McAllester.
Ten challenges in propositional reasoning and search.
Proceedings, 15th International Joint Conference on Artificial
Intelligence (IJCAI-97), 50--54. Morgan Kaufmann, 1997.

\bibitem{Sem08}
G. Semerjian,
 On the freezing of variables in random constraint satisfaction problems,
 J. Stat. Phys. 130 (2008) 251--293.

\bibitem{SeMo03}
G. Semerjian and R. Monasson,
Relaxation and metastability in a local search procedure
for the random satisfiability problem.
Phys.\ Rev.\ E 67 (2003) 066103.


\bibitem{BaHW03} W. Barthel, A. K. Hartmann, and M. Weigt,
Solving satisfiability problems by fluctuations: The dynamics
of stochastic local search algorithms.
{\it Phys. Rev. E 67} (2003), 066104.





\bibitem{Gu92} J. Gu,
Efficient local search for very large-scale satisfiability problems.
{\it SIGART Bulletin 3:1} (1992), 8--12.

\bibitem{Hoos02} H. H. Hoos,
An adaptive noise mechanism for WalkSAT.
{\it Proc.\ 18th Natl.\ Conf.\ on Artificial Intelligence (AAAI-02)},
655--660. AAAI Press, San Jose Ca, 2002.

\bibitem{HoSt99} H. H. Hoos and T. St\"utzle,
Towards a characterisation of the behaviour of stochastic local
search algorithms for SAT.
{\it Artificial Intelligence 112} (1999), 213--232.


\bibitem{MeZe02} M. M\'ezard and R. Zecchina,
Random K-satisfiability  problem: From an analytic solution
to an efficient algorithm.
{\it Phys. Rev. E 66} (2002), 056126.


\bibitem{Park02} A. J. Parkes,
Scaling properties of pure random walk on random 3-SAT.
{\it Proc.\ 8th Intl.\ Conf.\ on Principles and Practice
of Constraint Programming (CP 2002)}, 708--713.
Lecture Notes in Computer Science 2470.
Springer-Verlag, Berlin 2002.


\bibitem{SeKC96} B. Selman, H. Kautz, B. Cohen,
Local search strategies for satisfiability testing.
In: D. S. Johnson and M. A. Trick (Eds.),
{\it Cliques, Coloring, and Satisfiability}, 521--532.
DIMACS Series in Discr.\ Math.\ and Theoret.\ Comput.\ Sci. 26,
American Math.\ Soc., Providence RI, 1996.

\bibitem{SeLM92} B. Selman, H. J. Levesque, and D. G. Mitchell,
A new method for solving hard satisfiability problems.
{\it Proc.\ 10th Natl.\ Conf.\ on Artificial Intelligence (AAAI-92)},
440--446. AAAI Press, San Jose CA, 1992.

\bibitem{Sch02} U. Schoning,
A probabilistic algorithm for k-SAT based on limited local search and restart.
{\it Algorithmica 32} (2002), 615

\bibitem{SeMo03} G. Semerjian and R. Monasson,
Relaxation and metastability in a local search procedure
for the random satisfiability problem.
{\it Phys.\ Rev.\ E 67} (2003), 066103.


\bibitem{WeSe02} W. Wei and B. Selman,
Accelerating random walks.
{\it Proc.\ 8th Intl.\ Conf.\ on Principles and Practice
of Constraint Programming (CP 2002)}, 216--232.
Lecture Notes in Computer Science 2470.
Springer-Verlag, Berlin 2002.
